't Hooft surface operators in five dimensions and elliptic Ruijsenaars operators

We introduce codimension three magnetically charged surface operators in five-dimensional (5d) $\mathcal{N}=1$ supersymmetric gauge on $T^2 \times \mathbb{R}^3$. We evaluate the vacuum expectation values (vevs) of surface operators by supersymmetric localization techniques. Contributions of Monopole bubbling effects to the path integral are given by elliptic genera of world volume theories on D-branes. Our result gives an elliptic deformation of the SUSY localization formula \cite{Ito:2011ea} (resp. \cite{Okuda:2019emk, Assel:2019yzd}) of BPS 't Hooft loops (resp. bare monopole operators) in 4d $\mathcal{N}=2$ (resp. 3d $\mathcal{N}=4$) gauge theories. We define deformation quantizations of vevs of surface operators in terms of the Weyl-Wigner transform, where the $\Omega$-background parameter plays the role of the Planck constant. For 5d $\mathcal{N}=1^*$ gauge theory, we find that the deformation quantization of the surface operators in the anti-symmetric representations agrees with the type A elliptic Ruijsenaars operators. The mutual commutativity of these difference operators is related to the commutativity of products of 't Hooft surface operators.

==> README <==
YOUNGTAB-Package
================
-----------------------------------------------------------------------
Authors: 
-----------------------------------------------------------------------

Volker B"orchers (email: boercher@physik.uni-bremen.de)
and Stefan Gieseke (email: gieseke@physik.uni-bremen.de)

-----------------------------------------------------------------------
Legal stuff: 
-----------------------------------------------------------------------
Copyright (C) 1996,98,99 Volker B"orchers and Stefan Gieseke,
This program can be redistributed and/or modified under the terms
of the LaTeX Project Public License Distributed from CTAN
archives in directory macros/latex/base/lppl.txt; either
version 1 of the License, or any later version.

-----------------------------------------------------------------------
FILES:
-----------------------------------------------------------------------

README
---------------- the file you're reading now

youngtab.dtx
---------------- a documentated version of the package. From it you can
generate both a documentation and the .sty file without most comments
using the docstrip utility.

youngtab.ins
---------------- run TeX on it to generate the youngtab.sty in your
current working directory (from the .dtx file)

makeydoc
---------------- this (unix-) script generates youngtab.dvi, the
documentation for the package.

makeydoc.bat
---------------- same as makeydoc but for MSDOS (may need some editing).

gind.ist
---------------- You need it to generate the index for the
documentation. (gind.ist is a official part of doc/docstrip
package. Just in the case this is not installed...)

youngtab.tex
---------------- For thoose who don't use LaTeX but TeX.

youngtab.el
---------------- Only for thoose who use Emacs in connection with
AUC-TeX, the best TeX-shell i can imagine.. Makes life with
Young-Tableaux even easier (autocompletion, syntax help).


-----------------------------------------------------------------------
INSTALL:
-----------------------------------------------------------------------
1) `tex youngtab.ins' (alternatively: `latex youngtab.ins')
2) `makeydoc'
   * if you don't want any macrocode listings, uncomment the line
     containing ``\OnlyDescription'' (remove the `#')
3) put `youngtab.sty' to a path where LaTeX can find it.

-----------------------------------------------------------------------
For TeX-users:
-----------------------------------------------------------------------
follow the instructions in the documentation. (You must have
LaTeX2e to produce a .dvi file from youngtab.dtx -- Try to read the
.dtx file instead if you don't have!)
However there is a file already prepared for use with TeX:
`youngtab.tex' - try this and install in a directory where TeX will
find it.

-----------------------------------------------------------------------
For AUC-TeX-users:
-----------------------------------------------------------------------
. to install it once and for all, copy `youngtab.el' to the AUC-TeX
style-directory, e.g. /usr/lib/emacs/site-lisp/auctex/style/.
. to install it locally: do `mkdir style; cp youngtab.el style' in the
directory where your .tex files, using youngtab, reside (or in each if
you have more).
. Provides autocompletion and syntax checks for the switches and
dimensions "Y.*" and \young and \yng if you type `C-c RET' in emacs.

-----------------------------------------------------------------------
Date:
-----------------------------------------------------------------------
05/05/98

-----------------------------------------------------------------------
Version:
-----------------------------------------------------------------------
1.1


==> draft9/README <==
YOUNGTAB-Package
================
-----------------------------------------------------------------------
Authors: 
-----------------------------------------------------------------------

Volker B"orchers (email: boercher@physik.uni-bremen.de)
and Stefan Gieseke (email: gieseke@physik.uni-bremen.de)

-----------------------------------------------------------------------
Legal stuff: 
-----------------------------------------------------------------------
Copyright (C) 1996,98,99 Volker B"orchers and Stefan Gieseke,
This program can be redistributed and/or modified under the terms
of the LaTeX Project Public License Distributed from CTAN
archives in directory macros/latex/base/lppl.txt; either
version 1 of the License, or any later version.

-----------------------------------------------------------------------
FILES:
-----------------------------------------------------------------------

README
---------------- the file you're reading now

youngtab.dtx
---------------- a documentated version of the package. From it you can
generate both a documentation and the .sty file without most comments
using the docstrip utility.

youngtab.ins
---------------- run TeX on it to generate the youngtab.sty in your
current working directory (from the .dtx file)

makeydoc
---------------- this (unix-) script generates youngtab.dvi, the
documentation for the package.

makeydoc.bat
---------------- same as makeydoc but for MSDOS (may need some editing).

gind.ist
---------------- You need it to generate the index for the
documentation. (gind.ist is a official part of doc/docstrip
package. Just in the case this is not installed...)

youngtab.tex
---------------- For thoose who don't use LaTeX but TeX.

youngtab.el
---------------- Only for thoose who use Emacs in connection with
AUC-TeX, the best TeX-shell i can imagine.. Makes life with
Young-Tableaux even easier (autocompletion, syntax help).


-----------------------------------------------------------------------
INSTALL:
-----------------------------------------------------------------------
1) `tex youngtab.ins' (alternatively: `latex youngtab.ins')
2) `makeydoc'
   * if you don't want any macrocode listings, uncomment the line
     containing ``\OnlyDescription'' (remove the `#')
3) put `youngtab.sty' to a path where LaTeX can find it.

-----------------------------------------------------------------------
For TeX-users:
-----------------------------------------------------------------------
follow the instructions in the documentation. (You must have
LaTeX2e to produce a .dvi file from youngtab.dtx -- Try to read the
.dtx file instead if you don't have!)
However there is a file already prepared for use with TeX:
`youngtab.tex' - try this and install in a directory where TeX will
find it.

-----------------------------------------------------------------------
For AUC-TeX-users:
-----------------------------------------------------------------------
. to install it once and for all, copy `youngtab.el' to the AUC-TeX
style-directory, e.g. /usr/lib/emacs/site-lisp/auctex/style/.
. to install it locally: do `mkdir style; cp youngtab.el style' in the
directory where your .tex files, using youngtab, reside (or in each if
you have more).
. Provides autocompletion and syntax checks for the switches and
dimensions "Y.*" and \young and \yng if you type `C-c RET' in emacs.

-----------------------------------------------------------------------
Date:
-----------------------------------------------------------------------
05/05/98

-----------------------------------------------------------------------
Version:
-----------------------------------------------------------------------
1.1


==> draft9/makeydoc <==
#!/bin/sh
#
# Everything after a `#' is ignored (in this shell script)
#
# remove the string `> /dev/null' if you want more log-output
# remove the line containing `batchmode' if you want even more 
#  log-information while running LaTeX
#
#----------------- create a `ltxdoc.cfg': --------------------------

# Put here a list of options to pass to the class:
OPT=a4paper

echo "Generating configuration file ltxdoc.cfg for youngtab.dtx"

# Write the file in one pass:
cat > ltxdoc.cfg <<EOF
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ltxdoc.cfg for youngtab.dtx, generated by makeydoc %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\PassOptionsToClass{$OPT}{article}
\batchmode

%% Do not uncomment the next 2 lines
%\AtBeginDocument{\RecordChanges}
%\AtEndDocument{\PrintChanges}

%% The next 3 lines produce full indexes and change logs
%% - you may not want those (commented out by default).
\AtBeginDocument{\CodelineIndex\EnableCrossrefs}
\AtEndDocument{\PrintIndex}
\AtEndDocument{\addcontentsline{toc}{section}{Index}}

%% If you do not want any code listings, just documentation, then instead
%% of the lines above, uncomment the following:
%\AtBeginDocument{\OnlyDescription}
EOF
#---------- latex the documentation using `ltxdoc.cfg': --------------

ThisDoc=youngtab.dtx
Base=youngtab

echo;echo "1st latex $ThisDoc"
if (latex $ThisDoc > /dev/null) 
then
  echo;echo "2nd latex $ThisDoc"
  latex $ThisDoc > /dev/null

  echo;echo "makeindex -s gind.ist $Base.idx"
  makeindex -s gind.ist $Base.idx
  echo;echo "3rd latex $ThisDoc"
  latex $ThisDoc > /dev/null
else
  echo;cat <<EOF
  !!! LaTeX ERROR: $ThisDoc. (See $Base.log.)
  Perhaps a new version of youngtab.sty is missing?
  (Then, generate it by "tex youngtab.ins")
EOF
fi


==> makeydoc <==
#!/bin/sh
#
# Everything after a `#' is ignored (in this shell script)
#
# remove the string `> /dev/null' if you want more log-output
# remove the line containing `batchmode' if you want even more 
#  log-information while running LaTeX
#
#----------------- create a `ltxdoc.cfg': --------------------------

# Put here a list of options to pass to the class:
OPT=a4paper

echo "Generating configuration file ltxdoc.cfg for youngtab.dtx"

# Write the file in one pass:
cat > ltxdoc.cfg <<EOF
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ltxdoc.cfg for youngtab.dtx, generated by makeydoc %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\PassOptionsToClass{$OPT}{article}
\batchmode

%% Do not uncomment the next 2 lines
%\AtBeginDocument{\RecordChanges}
%\AtEndDocument{\PrintChanges}

%% The next 3 lines produce full indexes and change logs
%% - you may not want those (commented out by default).
\AtBeginDocument{\CodelineIndex\EnableCrossrefs}
\AtEndDocument{\PrintIndex}
\AtEndDocument{\addcontentsline{toc}{section}{Index}}

%% If you do not want any code listings, just documentation, then instead
%% of the lines above, uncomment the following:
%\AtBeginDocument{\OnlyDescription}
EOF
#---------- latex the documentation using `ltxdoc.cfg': --------------

ThisDoc=youngtab.dtx
Base=youngtab

echo;echo "1st latex $ThisDoc"
if (latex $ThisDoc > /dev/null) 
then
  echo;echo "2nd latex $ThisDoc"
  latex $ThisDoc > /dev/null

  echo;echo "makeindex -s gind.ist $Base.idx"
  makeindex -s gind.ist $Base.idx
  echo;echo "3rd latex $ThisDoc"
  latex $ThisDoc > /dev/null
else
  echo;cat <<EOF
  !!! LaTeX ERROR: $ThisDoc. (See $Base.log.)
  Perhaps a new version of youngtab.sty is missing?
  (Then, generate it by "tex youngtab.ins")
EOF
fi

